Estimating Conditional Mutual Information for Dynamic Feature Selection

Dynamic feature selection, where we sequentially query features to make accurate predictions with a minimal budget, is a promising paradigm to reduce feature acquisition costs and provide transparency into a model's predictions. The problem is challenging, however, as it requires both predicting with arbitrary feature sets and learning a policy to identify valuable selections. Here, we take an information-theoretic perspective and prioritize features based on their mutual information with the response variable. The main challenge is implementing this policy, and we design a new approach that estimates the mutual information in a discriminative rather than generative fashion. Building on our approach, we then introduce several further improvements: allowing variable feature budgets across samples, enabling non-uniform feature costs, incorporating prior information, and exploring modern architectures to handle partial inputs. Our experiments show that our method provides consistent gains over recent methods across a variety of datasets.

==> old/related.tex <==
% Nearly identical related work to previous paper. Only difference is discussing previous paper and variational information pursuit, which are early works on ``discriminative'' approaches.

% We briefly discuss works that has considered dynamic and static feature selection.

% \paragraph{Greedy CMI policies}

% \paragraph{Reinforcement learning}

% \paragraph{Static feature selection}


% An early work on the subject of
% One of the earliest works on DFS is \citet{fleuret2004fast}, who considered CMI as a selection criterion but only considered binary features.
One of the earliest works on DFS is \citet{geman1996active}, who used CMI as a selection criterion
% considered a selection criterion equivalent to the CMI
but made simplifying assumptions about the data distribution.
% provided an approximation only for binary features.
% only a crude approximation for binary features.
% , and even before this
% Before this, such
% Before this, information-theoretic principles were common in Bayesian experimental design \citep{lindley1956measure, bernardo1979expected}.
\citet{chen2015sequential} analyzed the greedy CMI approach theoretically
% from a theoretical perspective and showed 
and proved conditions under which it achieves near-optimal performance.
More recent works have focused
% recently, several works revisited the topic and focused 
% with a renewed focus
on practical implementations: among them, several focused on generative modeling approaches to approximate the CMI \citep{ma2019eddi, rangrej2021probabilistic, chattopadhyay2022interpretable, he2022bsoda}, and two
% concurrent
works
% others
proposed
% discriminative approaches that directly predict the optimal feature index
predicting the optimal feature index in a discriminative fashion \citep{chattopadhyay2023variational, covert2023learning}.
% feature index with maximum CMI \citep{chattopadhyay2023variational, covert2023learning}.
Our work develops a similar discriminative approach, but to estimate the CMI itself rather than the argmax among candidate features, which bypasses the need for training complex generative models.
% provides an
% we show that
% this offers
% a simpler
% and more accurate
% alternative to current generative approaches.
% discriminative approach that estimates the CMI itself, but in a way that is simpler and more accurate than current generative approaches.
% rather than its argmax,
% which is currently only possible with generative approaches,
% and explores capabilities that this enables.

Apart from these CMI-based methods,
% part of the literature,
% line of work,
other
% other
works have addressed DFS as an RL problem \citep{dulac2011datum, shim2018joint, kachuee2018opportunistic, janisch2019classification, janisch2020classification, li2021active}. For example, \citet{janisch2019classification} formulate DFS as a MDP
% Markov decision process (MDP)
where the reward is the 0-1 loss minus the feature cost, \revision{while considering both variable budgets and non-uniform feature costs}. RL theoretically has the capacity to discover better policies than a greedy approach, but it has not been found to perform well in practice 
% \citep{erion2021coai, chattopadhyay2023variational, covert2023learning}, 
seemingly due to training difficulties that are common in RL \citep{erion2021coai, chattopadhyay2023variational, covert2023learning}.
Other works have instead explored imitation learning, where selections are made by mimicking an oracle policy \citep{he2012cost, he2016active}.

Static
% (rather than dynamic)
feature selection has been an important subject in statistics and machine learning for decades; see \citep{guyon2003introduction, li2017feature, cai2018feature} for reviews. CMI is also at the basis of some static methods, see \citet{fleuret2004fast} for example. Greedy methods 
% have been proven to
perform well under certain assumptions about the data distribution \citep{das2011submodular, elenberg2018restricted}, and such methods are popular for models that are inexpensive to fit (e.g., linear regression). Feature selection with neural networks is more challenging, but methods now exist
% have been developed
that leverage either group sparse penalties \citep{feng2017sparse, tank2021neural, lemhadri2021lassonet} or differentiable gating mechanisms \citep{chang2017dropout, balin2019concrete, lindenbaum2021differentiable}.
Unlike recent DFS methods \citep{chattopadhyay2023variational, covert2023learning},
% Such gating approaches were the basis for recent DFS methods \citep{chattopadhyay2023variational, covert2023learning}, but 
our work bypasses these techniques by using a simpler regression objective.

\revision{Finally, mutual information estimation with deep learning has been an active topic in recent years. Unlike prior works \citep{oord2018representation, belghazi2018mutual, poole2019variational, song2019understanding, shalev2022neural}, ours focuses on the mutual information between features and a response variable, treats each feature separately, and can condition on arbitrary feature sets. Furthermore, while other methods train a model to estimate a single mutual information term, we accomplish this process via a predictive model that estimates the CMI in a single forward pass.}

